Online Learning with Sublinear Best-Action Queries

In online learning, a decision maker repeatedly selects one of a set of actions, with the goal of minimizing the overall loss incurred. Following the recent line of research on algorithms endowed with additional predictive features, we revisit this problem by allowing the decision maker to acquire additional information on the actions to be selected. In particular, we study the power of \emph{best-action queries}, which reveal beforehand the identity of the best action at a given time step. In practice, predictive features may be expensive, so we allow the decision maker to issue at most $k$ such queries. We establish tight bounds on the performance any algorithm can achieve when given access to $k$ best-action queries for different types of feedback models. In particular, we prove that in the full feedback model, $k$ queries are enough to achieve an optimal regret of $\Theta\left(\min\left\{\sqrt T, \frac Tk\right\}\right)$. This finding highlights the significant multiplicative advantage in the regret rate achievable with even a modest (sublinear) number $k \in \Omega(\sqrt{T})$ of queries. Additionally, we study the challenging setting in which the only available feedback is obtained during the time steps corresponding to the $k$ best-action queries. There, we provide a tight regret rate of $\Theta\left(\min\left\{\frac{T}{\sqrt k},\frac{T^2}{k^2}\right\}\right)$, which improves over the standard $\Theta\left(\frac{T}{\sqrt k}\right)$ regret rate for label efficient prediction for $k \in \Omega(T^{2/3})$.

==> sections/adversarial/old_adversarial_label_efficient.tex <==
\subsection{Label Efficient Query Model: An $O(\frac{T^2\log n}{k^2})$ Regret Bound} \label{app:hedgelim}

We extend Algorithm~\ref{alg:min-hedge} to a setting where feedback is given only during querying time steps, with the only difference that the update rule is performed just after the querying time steps and nowhere else across the time horizon. Namely, 
\[
    w_{t+1}(i) = \begin{cases}
        w_t(i) \cdot \exp{-\eta(\ell_t(i)-\ell_t(i^*_t))}, \text{ if } t \in Q\\
        w_t(i), \text{ otherwise}
    \end{cases}.
\]
The algorithm simply selects action $i$ with probability $p_t(i)$ for $t \in [T] \setminus Q$. We first observe the following:
\begin{observation}\label{obs:limfeed}
    For all $Q \subseteq [T], |Q|=k$, let $L_Q(i) = \sum_{t \in Q} \ell_t(i)$ and $L_Q^{\min} = \sum_{t \in Q} \ell_t(i^*_t)$ be defined analogously to $L_T(i), L_T^{\min}$. It holds that:
    \begin{align}
        \E{\substack{Q \subseteq [T]\\|Q|=k}}{\sum_{i \in [n], t \in [T] \setminus Q} p_t(i) \cdot \ell_t(i)} &= \frac{T-k}{k} \cdot \E{\substack{Q \subseteq [T]\\|Q|=k}}{\sum_{i \in [n], t \in Q} p_t(i) \cdot \ell_t(i)},\\
        L_T(i) &= \frac{T}{k} \cdot \E{\substack{Q \subseteq [T]\\|Q|=k}}{L_Q(i)},\\
        L_T^{\min} &=  \frac{T}{k} \cdot \E{\substack{Q \subseteq [T]\\|Q|=k}}{L_Q^{\min}},
    \end{align}
    where the expectation is over all uniformly random realizations of set $Q \subseteq [T]$ with $|Q|=k$.
\end{observation}

\begin{proof}[Proof of Theorem~\ref{thm:adv3}]
    We observe that the extension of Algorithm~\ref{alg:min-hedge} without queries to the label efficient query model, as described above, is again an instantiation $\Hedge(\tilde \bl, S)$ applied to losses $\tilde \ell_t(i) = \ell_t(i)-\ell_t(i^*_t)$ and $S = Q$, for every sampled random set $Q$. Then, Lemma~\ref{lem:potential-hedge} makes us conclude that, for every realization of set $Q$,
    \[
        \sum_{i \in [n], t \in Q} p_t(i) \cdot \ell_t(i) \leq \frac{L_Q(i)}{1-\eta} + \frac{\log n}{\eta(1-\eta)} - \frac{\eta L_Q^{\min}}{1-\eta}.
    \]
    Moreover, let us define 
    \[
        L_T(\cA_k \mid Q) = L_Q^{\min} + \sum_{i \in [n], t \in [T] \setminus Q} p_t(i) \cdot \ell_t(i),
    \]
    as the algorithm's expected loss conditioned on a specific realization of the random set $Q$. 
    %%%%%%%%%%%%%%%%%%%  Continua da qui
    Thus, by Observation~\ref{obs:limfeed}, we obtain 
    \begin{align*}
        L_T(\cA_k) &= \E{\substack{Q \subseteq [T]\\|Q|=k}}{L_T(\cA_k \mid Q)} = \E{\substack{Q \subseteq [T]\\|Q|=k}}{L_Q^{\min}} + \E{\substack{Q \subseteq [T]\\|Q|=k}}{\sum_{i \in [n], t \in [T] \setminus Q} p_t(i) \cdot \ell_t(i)}\\
        &\leq \frac{k}{T} \cdot L_T^{\min} + \frac{(1-\nicefrac{k}{T})\log n}{\frac{\eta k}{T}(1-\eta)} + \frac{(1-\nicefrac{k}{T}) L_T(i)}{1-\eta} - \frac{(1-\nicefrac{k}{T})\eta L_T^{\min}}{1-\eta}.
    \end{align*}
    Setting $\eta = \nicefrac{k}{T}$ yields $R_T(\cA_k) \leq \left(\frac{T}{k}\right)^2 \cdot \log n$.
\end{proof}

%%%%%%%%%%%% START - OLD PROOF OF HEDGE LABEL EFFICIENT
\iffalse
\begin{proof}[Proof of Theorem~\ref{thm:adv3}]
    We perform an almost identical analysis to the one in the proof of Theorem~\ref{thm:adv2}, which we illustrate below for completeness. We have that, by definition,
    \begin{align*}
        W_{T+1} \geq w_{T+1}(i) &= \begin{cases}
            w_T(i), &\text{ if } T \in [T] \setminus Q\\
            w_T(i) \cdot \exp{-\eta(\ell_t(i)-\ell_t(i^*_t))}, &\text{ otherwise}
        \end{cases} \\
        &= \prod_{t \in Q} \exp{-\eta(\ell_t(i)-\ell_t(i^*_t))} \\
        &= \exp{-\eta(L_Q(i)-L_Q^{\min})}.
    \end{align*}
    We also know that $W_{t+1} = W_t$ for all $t \in [T] \setminus Q$, and that otherwise
    \begin{align*}
        W_{t+1} &\leq W_t \cdot \left(1 - \eta\sum_{i \in [n]} p_t(i)\cdot(\ell_t(i)-\ell_t(i^*_t)) + \eta^2\sum_{i \in [n]} p_t(i)\cdot(\ell_t(i)-\ell_t(i^*_t))^2\right).
    \end{align*}
    Thus,
    \begin{align*}
        W_{T+1} &\leq n \cdot \prod_{t \in Q} \left(1 - \eta\sum_{i \in [n]} p_t(i)\cdot(\ell_t(i)-\ell_t(i^*_t)) + \eta^2\sum_{i \in [n]} p_t(i)\cdot(\ell_t(i)-\ell_t(i^*_t))^2\right),
    \end{align*}
    which combined with the earlier bound and taking logarithms of both sides, gives
    \begin{align*}
            &-\eta\left(L_Q(i)-L_Q^{\min}\right) \\
            &\leq \log n+\sum_{t \in Q} \log \left( 1 - \eta\sum_{i \in [n]} p_t(i)\cdot(\ell_t(i)-\ell_t(i^*_t)) +\eta^2\sum_{i \in [n]} p_t(i)\cdot( \ell_t(i)-\ell_t(i^*_t))^2 \right)\\
            &\leq \log n - \eta \sum_{t \in Q, i \in [n]} p_t(i)\cdot(\ell_t(i)-\ell_t(i^*_t)) + \eta^2\sum_{t \in Q, i \in [n]} p_t(i)\cdot(\ell_t(i)-\ell_t(i^*_t))^2\\
            &\leq \log n - (\eta - \eta^2) \sum_{t \in Q, i \in [n]} p_t(i)\cdot(\ell_t(i)-\ell_t(i^*_t)).
        \end{align*}
    The second inequality above follows from $\log(1+z) \leq z$ for $z \in \R$, and the third by observing that $(\ell_t(i)-\ell_t(i^*_t))^2 \leq \ell_t(i)-\ell_t(i^*_t)$, since $\ell_t(i^*_t) - \ell_t(i) \in [0,1]$. 
    This makes us conclude that for every realization of set $Q$,
    \[
        \sum_{i \in [n], t \in Q} p_t(i) \cdot \ell_t(i) \leq \frac{L_Q(i)}{1-\eta} + \frac{\log n}{\eta(1-\eta)} - \frac{\eta L_Q^{\min}}{1-\eta}.
    \]
    Moreover, let us define $$L_T(\cA_k \mid Q) = L_Q^{\min} + \sum_{i \in [n], t \in [T] \setminus Q} p_t(i) \cdot \ell_t(i),$$
    as the algorithm's expected loss conditioned on a specific realization of the random set $Q$. 
    %%%%%%%%%%%%%%%%%%%  Continua da qui
    Thus, by Observation~\ref{obs:limfeed}, we obtain 
    \begin{align*}
        L_T(\cA_k) &= \E{\substack{Q \subseteq [T]\\|Q|=k}}{L_T(\cA_k \mid Q)} = \E{\substack{Q \subseteq [T]\\|Q|=k}}{L_Q^{\min}} + \E{\substack{Q \subseteq [T]\\|Q|=k}}{\sum_{i \in [n], t \in [T] \setminus Q} p_t(i) \cdot \ell_t(i)}\\
        &\leq \frac{k}{T} \cdot L_T^{\min} + \frac{(1-\nicefrac{k}{T})\log n}{\frac{\eta k}{T}(1-\eta)} + \frac{(1-\nicefrac{k}{T}) L_T(i)}{1-\eta} - \frac{(1-\nicefrac{k}{T})\eta L_T^{\min}}{1-\eta}.
    \end{align*}
    Setting $\eta = \nicefrac{k}{T}$ yields $R_T(\cA_k) \leq \left(\frac{T}{k}\right)^2 \cdot \log n$.
\end{proof}
\fi
%%%%%%%%%%%% END - OLD PROOF OF HEDGE LABEL EFFICIENT

==> sections/adversarial/opt-adversary.tex <==
\subsection{Optimal Adversary against (Vanilla) Hedge with Uniform Querying}\label{sec:opt-adv}

We next show a lower bound on what the(vanilla) Hedge algorithm with uniform queries can guarantee. This is the same as the Adjusted Min-Hedge with Uniform Querying of \Cref{sec:hedge} but with update rule $w_{t+1}(i) = w_t(i) \cdot \exp{-\eta\ell_t(i)}$.\footnote{This is equivalent to an exponential update of $(1-\eta)^{\ell_t(i)}$.} Our goal is that of characterizing the optimal adversary for such algorithm similarly to \citet{GravinPS17}. We do so in multiple short claims to aid the understanding.

When two experts are considered, we can write the loss of the first expert as $\ell_t(1)$ and that of the second as $\ell_t(2) = \ell_t(1) + \varepsilon_t$ for some $\varepsilon_t \in [-1,1]$. Without loss of generality, assume that $L^*_T = \sum_{t \in [T]} \ell_t(1) \leq \sum_{t \in [T]} \ell_t(2)$: This directly implies that $\sum_{t \in [T]} \varepsilon_t \geq 0$. We also see that $L^{\min}_T = \sum_{t: \varepsilon_t > 0} \ell_t(1) + \sum_{t: \varepsilon_t \leq 0} (\ell_t(1) + \varepsilon_t) = L^*_T + \sum_{t: \varepsilon_t \leq 0} \varepsilon_t$. The regret can be simplified to
\[
    R_T(\cA) = L_T(\cA) - L^*_T = \left(1 - \frac{k}{T}\right) \cdot \left(\widetilde{L}_T(\cA) - L^*_T\right) + \frac{k}{T} \cdot \sum_{t: \varepsilon_t \leq 0} \varepsilon_t.
\]

\begin{proposition}\label{prop:reg-hedge}
    For all $\eta > 0$ and all instances composed of two experts, algorithm $\cA$, i.e., Hedge with learning rate $\eta$ and uniform querying $k$, suffers regret
    \begin{align*}
        R_T(\cA) = \left(1 - \frac{k}{T}\right) \cdot \sum_{t \in [T]} \varepsilon_t \cdot \frac{\exp{-\eta \sum_{\tau < t} \varepsilon_\tau}}{1 + \exp{-\eta \sum_{\tau < t} \varepsilon_\tau}} + \frac{k}{T} \cdot \sum_{t: \varepsilon_t \leq 0} \varepsilon_t.
    \end{align*}
\end{proposition}
\begin{proof}
    We write
    \begin{align*}
            \widetilde{L}_T(\cA) &= \sum_{t \in [T]} \frac{w_t(1) \cdot \ell_t(1) + w_t(2) \cdot \ell_t(2)}{W_t} \\
            &= \sum_{t \in [T]} \frac{\exp{-\eta\sum_{\tau < t} \ell_\tau(1)} \cdot \ell_t(1) + \exp{-\eta\sum_{\tau < t} \left(\ell_\tau(1)+\varepsilon_\tau\right)} \cdot \left(\ell_t(1)+\varepsilon_t\right)}{\exp{-\eta\sum_{\tau < t} \ell_\tau(1)} + \exp{-\eta\sum_{\tau < t} \left(\ell_\tau(1)+\varepsilon_\tau\right)}}\\
            &= \sum_{t \in [T]} \ell_t(1) + \sum_{t \in [T]} \varepsilon_t \cdot \frac{\exp{-\eta\sum_{\tau < t} \ell_\tau(1)} \cdot \exp{-\eta\sum_{\tau < t} \varepsilon_\tau}}{\exp{-\eta\sum_{\tau < t} \ell_\tau(1)} \cdot \left(1 + \exp{-\eta\sum_{\tau < t} \varepsilon_\tau}\right)}\\
            &= L^*_T + \sum_{t \in [T]} \varepsilon_t \cdot \frac{\exp{-\eta\sum_{\tau < t} \varepsilon_\tau}}{1 + \exp{-\eta\sum_{\tau < t} \varepsilon_\tau}} \\
            &= L^*_T + \sum_{t \in [T]} \varepsilon_t \cdot \frac{\exp{-\eta \Delta_t}}{1 + \exp{-\eta \Delta_t}},
        \end{align*}
        where we have denoted by $\Delta_t := \sum_{\tau < t} \varepsilon_\tau$ for all $t \geq 2$, and $\Delta_1 = 0$. Hence, the regret of Hedge with uniform querying reads
        \begin{align*}
            R_T(\cA) = \left(1 - \frac{k}{T}\right) \cdot \sum_{t \in [T]} \varepsilon_t \cdot \frac{\exp{-\eta \Delta_t}}{1 + \exp{-\eta \Delta_t}} + \frac{k}{T} \cdot \sum_{t: \varepsilon_t \leq 0} \varepsilon_t.
        \end{align*}
        This concludes the proof.
\end{proof}

From the proof, we notice that the adversary's task simply reduces to choose $\varepsilon_t$'s so as to maximize the regret expression: Choosing them to be all non-negative can only help the learner, as the next proposition shows.
\begin{proposition}\label{prop:reg-hedge-pos}
    For all $\eta > 0$ and all instances composed of two experts, algorithm $\cA$, i.e., Hedge with learning rate $\eta$ and uniform querying $k$, suffers regret at most $R_T(\cA) \leq 1+ \frac{\log(T)}{\eta}$, if all $\varepsilon_t \geq 0$.
\end{proposition}
\begin{proof}
    Given that all $\varepsilon_t \geq 0$, then $\Delta_t \leq \Delta_{t+1}$. Let $r$ be the last time step $t$ such that $\Delta_t \leq 1$. Then, using the equality established in \Cref{prop:reg-hedge}, we get
        \begin{align*}
            R_T(\cA) \leq \sum_{t \leq r} \varepsilon_t \cdot \frac{\exp{-\eta \Delta_t}}{1 + \exp{-\eta \Delta_t}} + \sum_{t > r} \varepsilon_t \cdot \frac{\exp{-\eta \Delta_t}}{1 + \exp{-\eta \Delta_t}}    \leq S_{r+1} + \frac{1}{\eta} \cdot \sum_{t > r} \frac{\varepsilon_t}{\Delta_t} \leq 1+ \frac{\log(T-r)}{\eta},
        \end{align*}
        where the second inequality follows from $\frac{\exp{\cdot}}{1+\exp{\cdot}} \leq 1$, the definition of $S_{r+1}$, and the fact that $\frac{\exp{-\eta \Delta_t}}{1 + \exp{-\eta \Delta_t}} \leq \frac{1}{\eta \Delta_t}$, for all $\Delta_t \geq 1$. The last inequality is obtained via the following inductive argument: First, note that, for all $t > r+1$, $\frac{\varepsilon_t}{\Delta_t} \leq \frac{\varepsilon_t}{1+\varepsilon_{r+1}+\ldots+\varepsilon_{t-1}}$, and $\frac{\varepsilon_{r+1}}{S_{r+1}} \leq \varepsilon_{r+1}$. Second, the adversary could set $\varepsilon_T = 1$ as this would be the optimal way to increase the sum. Given these two facts, we have the following upper bound:
        \[
            \sum_{t > r} \frac{\varepsilon_t}{\Delta_t} \leq \varepsilon_{r+1} + \frac{\varepsilon_{r+2}}{1+\varepsilon_{r+1}} + \ldots + \frac{\varepsilon_{T-1}}{1+\varepsilon_{r+1}+\ldots+\varepsilon_{T-2}} + \frac{1}{1+\varepsilon_{r+1}+\ldots+\varepsilon_{T-1}}.
        \]
        We observe $\varepsilon_t$ only appears in the numerator of ratio $t$ and in all denominators of ratios starting at $t+1$ until the last. This means that, starting at $T-1$, and given that all $\varepsilon_t \geq 0$, the adversary should set $\varepsilon_{T-1} = 1$, as it maximizes the expression. Backwards, for $\varepsilon_t$, the adversary has to maximize
        \[
            \frac{\varepsilon_t}{1+C} + \frac{1}{1+C+\varepsilon_t} + \frac{1}{2+C+\varepsilon_t} + \ldots + \frac{1}{T-t+C+\varepsilon_t},
        \]
        where $C = \varepsilon_{r+1}+\ldots+\varepsilon_{t-1}$. This is maximized at $\varepsilon_t=1$ as $C \geq 0$. Thus, all $\varepsilon_t$'s are set to $1$ and we obtain
        \[
            \sum_{t > r} \frac{\varepsilon_t}{\Delta_t} \leq 1 + \frac{1}{2} + \ldots + \frac{1}{T-r} \leq \log(T-r),
        \]
        which yields the claim.
\end{proof}
We stress that the above proposition does not depend on the amount of querying, and it is true even in the absence of queries. This proposition motivates us to characterize structural properties of the optimal adversary against Hedge, which we do in the next section.

We state the following two straightforward observations:
\begin{observation}
    Given a specific (possibly randomized) algorithm, or family of parametrized algorithms, the structure of the optimal adversary can \emph{always} be found among deterministic strategies.
\end{observation}

\begin{observation}\label{obs:probs}
    When the number of experts is $m=2$, assuming the total gap between expert 1 and expert 2 is $\Delta_t$ at time step $t$, Hedge (without querying) selects expert 1 (the leading expert) with probability $\frac{\exp{\eta \Delta_t}}{1+\exp{\eta \Delta_t}}$, and expert 2 (the following expert) with probability $\frac{1}{1+\exp{\eta \Delta_t}}$. When Hedge also possesses a Uniform Querying power of cardinality $k$, then it selects the leading expert with probability $\frac{k}{T} + \left(1 - \frac{k}{T}\right) \cdot \frac{\exp{\eta \Delta_t}}{1+\exp{\eta \Delta_t}}$, and the following expert with probability $\frac{k}{T} + \left(1 - \frac{k}{T}\right) \cdot \frac{1}{1+\exp{\eta \Delta_t}}$. Therefore, Hedge (with or without uniform querying) bases its decision solely depending on the value of $\Delta_t$.
\end{observation}

In what follows, the plan is to show that the adversary changes the gap between leading and following expert by some $\varepsilon_t$ at each time step. Moreover, the adversary has no incentive to increase the gap for an arbitrary number of steps, then decrease it, to increase it again in a ``disconnected'' manner. It is always more effective for the adversary to loop between an increase of $\varepsilon_t$ and a decrease of $\varepsilon_{t+1}$ for a certain number of steps, to then increase the gap between the two experts by $\varepsilon_t$ for each of the remaining steps.

Following \citet{GravinPS17}, we refer to the \emph{looping phase} as the sequence of time steps where the adversary sets $\Delta_{t+1}=\Delta_t+\varepsilon_{t+1}, \Delta_{t+2}=\Delta_{t+1}+\varepsilon_{t+2}$, where $\varepsilon_{t+2} \leq 0 \leq \varepsilon_{t+1}$, for all $t \leq T - \widetilde{T}$ and some even integer $0\leq \widetilde{T} \leq T$. Similarly, we refer to the \emph{increasing phase} to the sequence of time steps where the adversary sets $\Delta_{t+1}=\Delta_t+\varepsilon_{t+1}$ for all $t > T - \widetilde{T}$. Finally, we denote by $R^{\looping}_T(\cA), R^{\incr}_T(\cA)$ the regret incurred by Hedge respectively on the looping phase, and on the increasing phase.

A key ingredient in the analysis is that, for all $t \in [T]$, the change in regret to due a change in $\Delta_t$ is independent of the time step $t$. This, together with the consideration that it is best to loop either at the start or at the end, implies that the optimal adversarial strategy is to split the time horizon in a looping phase $t \leq T - \widetilde{T}$ and in an increasing phase $t > T - \widetilde{T}$, or vice versa. 

Formally, we prove the following results:

\begin{lemma}[Structure of the Optimal Adversary, adaptation of Section 2 in \cite{GravinPS17}]\label{lem:opt-adv}
    Consider $m=2$ experts, a fixed $\eta > 0$, and some even integer $0\leq \widetilde{T} \leq T$. The optimal adversarial structure against Hedge with Uniform Querying is the following: (1) Perform a looping phase of length $\frac{T - \widetilde{T}}{2}$, then (2) perform an increasing phase for the remaining $\widetilde{T}$ steps, or vice versa. 
\end{lemma}

\begin{proof}
    We note that the regret inflicted due to an increase of $\Delta_{t-1}$ by $\varepsilon_t$ is $\frac{1 - \frac{k}{T}}{1+\exp{\eta \Delta_{t-1}}} \cdot \varepsilon_t$, since the leading expert increases its value by $\varepsilon_t$ but $\cA$ only selects the leading expert with probability $\frac{k}{T} + \left(1 - \frac{k}{T}\right) \cdot \frac{\exp{\eta \Delta_{t-1}}}{1+\exp{\eta \Delta_{t-1}}}$, as per \Cref{obs:probs}. 
    
    On the other hand, a decrease of $\Delta_t$ by $\varepsilon_{t+1}$ inflicts a regret of $- \frac{1 + \frac{k}{T} \cdot \exp{\eta \Delta_t}}{1+\exp{\eta \Delta_t}} \cdot \varepsilon_{t+1}$, since the leading expert's value remains unaltered while the following expert's value increases by $\varepsilon_{t+1}$ and is selected by $\cA$ with probability $\frac{k}{T} + \left(1 - \frac{k}{T}\right) \cdot \frac{1}{1+\exp{\eta \Delta_t}}$, again by \Cref{obs:probs}.
    
    To show that it is always beneficial for the looping phase to precede the increasing phase, let us make the following considerations. First, we have that the change in regret is independent of time, so that combining the looping steps together and the increasing steps steps together is a weakly dominant strategy for the adversary. Moreover, note that the regret inflicted by a looping step (i.e., $\Delta_{t-1} \rightarrow \Delta_{t-1} + \varepsilon_t \rightarrow \Delta_{t-1} + \varepsilon_t + \varepsilon_{t+1}$, with $\varepsilon_{t+1} \leq 0 \leq \varepsilon_t$) is
    \[
        \frac{1 - \frac{k}{T}}{1+\exp{\eta \Delta_{t-1}}} \cdot \varepsilon_t - \frac{1 + \frac{k}{T} \cdot \exp{\eta (\Delta_{t-1}+\varepsilon_t)}}{1+\exp{\eta (\Delta_{t-1}+\varepsilon_t)}} \cdot \varepsilon_{t+1}.
    \]
    The above expression is either maximized at $\Delta_{t-1} = 0$, if , or otherwise at $\Delta_{t-1} = T$, for all $k \leq T, \eta > 0$. Hence, the adversary first performs all $\frac{T - \widetilde{T}}{2}$ loops, and the $\widetilde{T}$ increasing steps right after, or vice versa.
\end{proof}

\mr{Observe that any other value between $-1$ and $1$ (including $0$) only scales down the size of the inflicted regret at each time step. Therefore, in both the looping and the increasing phase, the adversary is better off increasing or decreasing the gap by exactly 1.}

\begin{theorem}\label{thm:reg-hedge}
    Algorithm $\cA$, i.e., Hedge with learning rate $\eta = \max\left\{\frac{1}{\sqrt{T}}, \frac{k}{T}\right\}$ and uniform querying $k$, suffers regret
    \begin{align*}
        R_T(\cA) \leq ,
    \end{align*}
    all instances composed of two experts.
\end{theorem}
\begin{proof}
    We know that $R_T(\cA) = R^{\looping}_T(\cA) + R^{\incr}_T(\cA)$, thus we proceed to bound them separately. From the proof of \Cref{lem:opt-adv}, we know that the maximum regret is inflicted by performing $\frac{T-\widetilde{T}}{2}$ loops at $\Delta=0$, so that by simplifying, we obtain
    \[
        R^{\looping}_T(\cA) = \frac{T-\widetilde{T}}{2} \cdot \left(\frac{1 - \frac{k}{T}}{2} -\frac{1 + \frac{k}{T} \cdot \exp{\eta}}{1+\exp{\eta}}\right) \leq \frac{T-\widetilde{T}}{4} \cdot \frac{\left(1 - \frac{2k}{T}\right)\cdot \exp{\eta}-1}{\exp{\eta}+1}.
    \]
    On the other hand,
    \begin{align*}
        R^{\incr}_T(\cA) &= \left(1-\frac{k}{T}\right) \cdot \sum_{\Delta=0}^{\widetilde{T}-1} \frac{1}{1+\exp{\eta\Delta}} \leq \left(1-\frac{k}{T}\right) \cdot \int_{0}^{\widetilde{T}} \frac{d\Delta}{1+\exp{\eta \Delta}}\\
        &= \left(1-\frac{k}{T}\right) \cdot \frac{1}{\eta} \cdot \log\left(\frac{2\cdot\exp{\eta\widetilde{T}}}{1+\exp{\eta\widetilde{T}}}\right) \leq \frac{1}{\eta} \cdot \log\left(\frac{2\cdot\exp{\eta\widetilde{T}}}{1+\exp{\eta\widetilde{T}}}\right).
    \end{align*}
    Since both regret terms are concave in $\widetilde{T}$ (so, their sum is too), it suffices to consider $\widetilde{T}=0, \widetilde{T}=T$ and the $\widetilde{T}$ selected by setting the derivatives on $R^{\looping}_T(\cA), R^{\incr}_T(\cA)$ upper bounds to $0$, to understand what the worst case in terms of $\widetilde{T}$ is. Recall that the learning rate is set to be $\eta = \max\left\{\frac{1}{\sqrt{T}}, \frac{k}{T}\right\}$.

    \paragraph{Case 1: $\widetilde{T}=0$.} We have that $R^{\incr}_T(\cA)=0$ and
    \[
        R_T(\cA) = R^{\looping}_T(\cA) \leq \frac{T}{4} \cdot \frac{\left(1 - \frac{2k}{T}\right)\cdot\exp{\eta}-1}{\exp{\eta}+1} \leq 
        \begin{cases}
            \frac{\sqrt{T}}{4}, &\text{ if } k \leq \sqrt{T}\\
            0, &\text{ otherwise}
        \end{cases}.
    \]

    \paragraph{Case 2: $\widetilde{T}=T$.} We have that $R^{\looping}_T(\cA)=0$ and \[
        R_T(\cA) = R^{\incr}_T(\cA) \leq \frac{1}{\eta} \cdot \log\left(\frac{2\cdot\exp{\eta T}}{1+\exp{\eta T}}\right) \leq \log(2) \cdot 
        \begin{cases}
            \sqrt{T}, &\text{ if } k \leq \sqrt{T}\\
            \frac{T}{k}, &\text{ otherwise}
        \end{cases}.
    \]

    \paragraph{Case 3: $0 < \widetilde{T} < T$.} We compute the derivative of (the upper bound on) $R_T(\cA)$ with respect to $\widetilde{T}$ from the two pieces composing it, $R^{\looping}_T(\cA)$ and (the upper bound on) $R^{\incr}_T$ and equate to 0. We have
    \begin{align*}
         \frac{1}{1+\exp{\eta\widetilde{T}}} - \frac{\left(1-\frac{2k}{T}\right)\cdot\exp{\eta} - 1}{4(\exp{\eta}+1)} = 0,
    \end{align*}
    which yields
    \begin{align*}
        \widetilde{T} = \frac{1}{\eta} \cdot \log\left(\frac{\left(3+\frac{2k}{T}\right)\cdot\exp{\eta}+5}{\left(1-\frac{2k}{T}\right)\cdot\exp{\eta}-1}\right).
    \end{align*}
    Plugging this value in the regret expressions of above, we get
    % \begin{align*}
    %     - \frac{\left(1-3\beta\right)\cdot\exp{\eta} - \left(1+\beta\right)}{4(1+\exp{\eta})} + \frac{1-\beta}{1+\exp{\eta\widetilde{T}}}.
    % \end{align*}
    % Equating this sum to 0, we obtain
    % \begin{align*}
    %     \widetilde{T} = \frac{1}{\eta} \cdot \log\left(\frac{(3-\beta)\cdot\exp{\eta} + (5-3\beta)}{(1-3\beta)\cdot\exp{\eta} - (1+\beta)}\right).
    % \end{align*}
    % Plugging this value in the regret expressions of above, we get
\end{proof}

==> sections/mab/upper-bound.tex <==
\subsection{An Online Learner in Full-feedback} \label{sec:ub-full}

In this section, we present an online learner $\cA$ with full-feedback which achieves a regret that gracefully degrades as the number of queries $k$ increases.

\paragraph{Algorithm.} The algorithm proceeds as follows at round $t$: Let $a_t \in [m]$ the arm maximizing the cumulative average reward (from the beginning), i.e.,
    \[
        a_t = \arg\max_{a \in [m]} \frac{1}{t-1} \cdot \sum_{s \in [t-1]} x_{a,s}.
    \]
\begin{itemize}
    \item If $t \leq k$ rounds, make a query, observe $\max_{a \in [m]} x_{a,t}$, and select the corresponding arm.
    \item Otherwise, select $a_t$.
\end{itemize}

The goal is to show that the above algorithm achieves the following guarantee:
\begin{theorem}\label{thm:stoch}
    Let $\bx \sim \cD^T$ be $T$ reward vectors (one component per arm) drawn from distribution $\cD = \bigtimes_{a \in [m]} \cD_a$. Then, algorithm $\cA$ with query access $k$ guarantees
    \[
        (k, R_T(\cA)) \lesssim \left(k, \min\left\{\sqrt{T\log\left(m\right)}, \frac{T\log\left(m\right)}{k}\right\}\right),
    \]
    with probability at least $1-\delta$.
\end{theorem}

\paragraph{Analysis.} The proof of \Cref{thm:stoch} is articulated in multiple short claims that make the exposition clearer.\footnote{See exercises in \url{https://web.stanford.edu/class/cs229t/2015/hw2.pdf}.}

\begin{fact}[Bernstein Concentration Inequality \cite{BoucheronLM13}]\label{fact:bernstein-simple}
    Let $Z_1, \ldots, Z_n$ be $n$ independent random variables with support $[0,1]$, expectation $\E{}{Z_i} = \mu$ and variance $\V{}{Z_i} = \sigma^2$, for all $i \in [n]$. We have
    \[
        \P{}{\frac{1}{n} \cdot \sum_{i \in [n]} Z_i - \mu > \varepsilon} \leq \exp{-\frac{3n\varepsilon^2}{6\sigma^2 + 2\varepsilon}}.
    \]
\end{fact}

\begin{claim}\label{cl:concentration}
    For all $t \in [T]$, consider the $a_t$ and the empirical reward $\barmu_t(a)$ of any arm $a \in [m]$. We have the following inequalities:
    \begin{enumerate}
        \item For all $a \in [m]$ such that $\mu(a) \leq \Psi$, $\P{}{\barmu_t(a) - \mu(a) > \varepsilon} \leq \exp{-\frac{3t\varepsilon^2}{6\Psi + 2\varepsilon}}$;
        \item For all $a^\prime \in [m]$ such that $\mu(a^\prime) > \Psi^\prime + \varepsilon$, $\P{}{\barmu_t(a^\prime) \leq \Psi^\prime} \leq \exp{-\frac{3t\varepsilon^2}{6\Psi^\prime + 8\varepsilon}}$;
        \item $\P{}{\mu(a^*) - \mu(a_t) > 2\varepsilon} \leq m \cdot \exp{-\frac{3t\varepsilon^2}{6\Psi + 14\varepsilon}}$.
    \end{enumerate}
\end{claim}
\begin{proof}
    The proof of the first two statements is direct from \Cref{fact:bernstein-simple}.
\end{proof}

We are now ready to prove the main theorem.

\begin{proof}[Proof of \Cref{thm:stoch}]
    We first observe that the number of mistakes $\cA$ makes in the first $k$ rounds is $0$, since it queries the true label. Hence, by \Cref{cl:concentration}, with probability at least $1 - \delta$, we have
    \begin{align*}
        R_T(\cA) = & -k\cdot(M - \mu(a^*)) + \sum_{t>k} \Delta(a_t) \\
        \leq &- k\Psi + \sum_{t>k} \left(10 \cdot \frac{\log\left(m\right) + \log\left(\frac{1}{\delta}\right)}{t} + 4\Psi^{\frac{1}{2}} \cdot \sqrt{\frac{\log\left(m\right) + \log\left(\frac{1}{\delta}\right)}{t}}\right) \\
        \leq &- k\Psi + 10\log(T)\cdot\left(\log(m) + \log\left(\frac{1}{\delta}\right)\right) + 8\sqrt{\Psi T\left(\log(m) + \log\left(\frac{1}{\delta}\right)\right)}.
    \end{align*}
    Let us put $k = T^\alpha$ and we let $\Psi = T^{-\beta}$, where $\alpha \in [0,1]$ and $\beta \geq 0$. Then, the regret can be upper bounded by
    \[
        R_T(\cA) \leq -T^{\alpha-\beta} + 10\log(T)\cdot\left(\log(m) + \log\left(\frac{1}{\delta}\right)\right) + 8\sqrt{T^{1-\beta}\left(\log(m) + \log\left(\frac{1}{\delta}\right)\right)}.
    \]
    In order to characterize the worst case, let $\beta = \beta(\alpha)$ be a function of $\alpha$.  We get that, to maximize the above expression, $\beta(\alpha) \simeq \max\left\{0, 2\alpha-1-\frac{\log\log(T)}{\log(T)}\right\}$. Thus,
    \begin{align*}
        R_T(\cA) &\lesssim \begin{cases}
            T^{\frac{1}{2}}\cdot \sqrt{\log(T)} - T^\alpha, &\text{ if } \alpha \lesssim \frac{1}{2} + \frac{\log\log(T)}{2\log(T)}\\
            T^{1-\alpha+\frac{\log\log(T)}{2\log(T)}} \cdot \sqrt{\log(T)} - T^{1-\alpha+\frac{\log\log(T)}{\log(T)}}, &\text{ otherwise }
        \end{cases}
        \\
        &\lesssim \begin{cases}
            \sqrt{T\log(T)}, &\text{ if } \alpha \lesssim \frac{1}{2} + \frac{\log\log(T)}{2\log(T)}\\
            T^{1-\alpha} \cdot \log(T), &\text{ otherwise }
        \end{cases} .
    \end{align*}
    This means that the bicriteria guarantee of algorithm $\cA$ reads
    \[
        (k, R_T(\cA)) \lesssim \left(k, \min\left\{\sqrt{T\log(m)}, \frac{T\log(m)}{k}\right\}\right),
    \]
    where we have substituted again $k = T^\alpha$.
\end{proof}



\subsection{An Online Learner in Bandit-feedback} \label{sec:ub}

We present our algorithm next.

\paragraph{Algorithm.} Our algorithm $\cA$ operates in two phases: In phase 1, it simply looks at all arms' rewards for the first $k$ rounds and pulls the arm with highest \emph{realized} reward at each round. For the remaining $T-k$ rounds, phase 2, the algorithm 
% performs one of the following two subroutines depending on quantity 
% \begin{align*}
%     \hat{\Psi} := \frac{1}{k} \cdot \left(\sum_{t \leq k} \max_{a \in [m]} x_{a,t} - \max_{a \in [m]} \sum_{t \leq k} x_{a,t}\right) \geq 0,
% \end{align*}
% where $\hat{\Psi}$ is an estimator of the (additive) gap between best dynamic policy and best arm in hindsight in the first $k$ rounds (i.e., respectively, expected maximum and maximum of expectations). We denote as $\hat{a}$ the arm maximizing the second sum above. If $\hat{\Psi} \lesssim \poly^{-1}(\log T)$, then we pull arm $\hat{a}$ until the end (so, for the $T-k$ remaining rounds), phase 2a. Otherwise, in phase 2b, the algorithm 
plays $\UCBone$ with $n_t(a)$'s initialized to $k$ (i.e., $n_k(a)=k$ for all $a \in [m]$), that is, it pulls the arm $a_t$ that minimizes
\[
    \UCB_t(a) = \barmu_{t}(a) + r_t(a), ~\forall a \in [m],
\]
where $\barmu_{t}(a) = \frac{1}{n_t(a)} \cdot \sum_{s \leq t} x_t(a)$, and $r_t(a) \geq 0$ to be derived later. 

\paragraph{Analysis.} We first note that, in phase 1, the algorithm gets in expectation the maximum reward from those rounds, i.e., 
\[
    \sum_{t \leq k} \E{\bx_t \sim \cD}{\max_{a \in [m]} x_{a,t}} = k\E{}{\max_{a \in [m]} x_a} =: kM.
\]

On the other hand, in phase 2, $\cA$ gets a reward equal to $\sum_{t>k} \mu(a_t)$. The regret is
\begin{align*}
    R_T(\cA) &= T\mu(a^*) - \sum_{t \in [T]} \mu(a_t) = -k\cdot(M - \mu(a^*)) + \sum_{t>k} \Delta(a_t).
\end{align*}
% \footnote{\citet{HillK81} also prove that $\Psi \leq \frac{1}{4}$ for independent random variables over $[0,1]$.} 
% Ideally, if we knew $\Psi$ exactly, we would split the analysis into two cases: $\Psi \lesssim \poly^{-1}(\log T)$, and otherwise. In the first case, we would know (with high probability) which arm is the best, incurring small regret. Otherwise, the UCB analysis would give us constant regret. However, we do not know $\Psi$ exactly, but we only have an estimate of it, $\hat{\Psi}$, and thus branch to cases based on this estimate. Our first step in the analysis is to bound the probability of branching to the ``wrong'' part of the algorithm, i.e., the probability that we overstimate $\Psi$ when we should fully exploit, or underestimate $\Psi$ when we should use UCB1.

% \paragraph{Concentration around $\Psi$.} To bound the error probability, we first make the following observations:
% \begin{observation}
%     Let $\overline{\Psi} := \E{}{\max_{a \in [m]} \frac{1}{k} \cdot \sum_{t \leq k} x_{a,t}} - M$ and $\alpha > 0$. We have that
%     \begin{enumerate}
%         \item $\E{}{\hat{\Psi}} \neq \Psi$, but $\E{}{\hat{\Psi}} = \overline{\Psi}$;
%         \item $\P{}{\hat{\Psi} - \Psi \geq \alpha} \leq \P{}{\hat{\Psi} - \overline{\Psi} \geq \alpha}$.
%     \end{enumerate}
% \end{observation}
% \begin{proof}
%     The first claim follows by definition. For the second claim, we have that
%     \begin{align*}
%         \hat{\Psi} - \Psi &= \frac{1}{k} \cdot \left(\sum_{t \leq k} \max_{a \in [m]} x_{a,t} - \max_{a \in [m]} \sum_{t \leq k} x_{a,t}\right) - M + \mu(a^*) \\
%         &= \left(\frac{1}{k} \cdot \sum_{t \leq k} \max_{a \in [m]} x_{a,t} - M \right) - \left(\frac{1}{k} \cdot \max_{a \in [m]} \sum_{t \leq k} x_{a,t} - \E{}{\max_{a \in [m]} \frac{1}{k} \cdot \sum_{t \leq k} x_{a,t}}\right) \\
%         &+ \underbrace{\left(\mu(a^*) - \E{}{\max_{a \in [m]} \frac{1}{k} \cdot \sum_{t \leq k} x_{a,t}}\right)}_{\leq 0} \\
%         &\leq \hat{\Psi} - \overline{\Psi},
%     \end{align*}
%     which concludes the proof.
% \end{proof}

% Equipped with the above observation, it suffices to study the concentration around $\overline{\Psi}$ rather than $\Psi$ itself. To this end, let us define self-bounding functions and state their desirable properties.
% \begin{definition}[Self-bounding functions]\label{def:bounding}
%     Let $\bZ = (Z_1, \ldots, Z_n)$ be a vector of $n$ independent random variables, and $\cZ$ the corresponding product space. Similarly, let $\bZ^{(i)} = (Z_1, \dots, Z_{i-1}, Z_{i+1}, \dots, Z_{n})$ be the same vector deprived of the $i^{\text{th}}$ coordinate, and $\cZ^{(i)}$ the corresponding product space. A function $g: \cZ \rightarrow \R$ is said to be self-bounding if there exists a series of functions $\{g_i\}_{1\leq i\leq n}$, such that each $g_i: \cZ^{(i)} \rightarrow \R$ satisfies 
%     \begin{align*}
%         0 \leq g(\bZ) - g_i(\bZ^{(i)}) &\leq 1,\\
%         \sum_{i \in [n]}{\left(g(\bZ) - g_i(\bZ^{(i)})\right)} &\leq g(\bZ).
%     \end{align*}
% \end{definition}

% \begin{proposition}\label{prop:deltahat-selfbdd}
%     Let $k \geq 1$ be an integer and let $\cX = [0,1]^m$. For $\hat{\Psi}: \cX^k \rightarrow \R_{\geq 0}$ defined as
%     \begin{align*}
%     \hat{\Psi}(\bX) := \frac{1}{k} \cdot \left(\sum_{t \leq k} \max_{a \in [m]} x_{a,t} - \max_{a \in [m]} \sum_{t \leq k} x_{a,t}\right),
% \end{align*}
% where $\bX = (\bx_t)_{t \leq k}$, $\bx_t \in \cX$, each with coordinates $x_{a,t} \in [0,1]$, for all $t \leq k$ and all $a \in [m]$. Then, $k\hat{\Psi}$ is self-bounding.
% \end{proposition}
% \begin{proof}
%     For all $i \leq k$, let $\hat{\Psi}_i: \left(\cX^k\right)^{(i)} \rightarrow \R_{\geq 0}$ be defined as
%     \begin{align*}
%         \hat{\Psi}_i(\bX^{(i)}) := \frac{1}{k} \cdot \left(\sum_{t \leq k: t \neq i} \max_{a \in [m]} x_{a,t} - \max_{a \in [m]} \sum_{t \leq k: t \neq i} x_{a,t}\right),
%     \end{align*}
%     and consider the sequence of functions $(k\hat{\Psi}_i)_{i\leq k}$. We have that, on all $\bX$,
%     \begin{align*}
%         0 \leq k\hat{\Psi}(\bZ) - k\hat{\Psi}_i(\bZ^{(i)}) &=  \max_{a \in [m]} x_{a,i} + \underbrace{\max_{a \in [m]} \sum_{t \leq k: t \neq i} x_{a,t} - \max_{a \in [m]} \sum_{t \leq k} x_{a,t}}_{\leq 0} \leq \max_{a \in [m]} x_{a,i} \leq 1,
%     \end{align*}
%     which proves the first property in \Cref{def:bounding}. For the second property, we have 
%     \begin{align*}
%         \sum_{i \leq k} \left(k\hat{\Psi}(\bZ) - k\hat{\Psi}_i(\bZ^{(i)})\right) &= \sum_{i \leq k} \left(\max_{a \in [m]} x_{a,i} + \max_{a \in [m]} \sum_{t \leq k: t \neq i} x_{a,t} - \max_{a \in [m]} \sum_{t \leq k} x_{a,t}\right)\\
%         &\leq \sum_{t \leq k} \max_{a \in [m]} x_{a,t} - \max_{a \in [m]} \sum_{t \leq k} x_{a,t} = k\hat{\Psi}(\bX),
%     \end{align*}
%     where the first inequality follows from difference-of-max being at most max-of-difference, while the second simply by observing (again by Jensen's Inequality) that $\sum_{i \leq k}$
% \end{proof}

% \begin{lemma}[Theorem 1 in \citep{BoucheronLM00}]\label{lem:blm}
% For a self-bounding function $g: \cZ \to \R$, it holds that:
% \begin{eqnarray*}
%     \mbox{\emph{For every }} \alpha>0, \qquad & \P{}{g(\bZ) \geq \E{}{g(\bZ)} + \alpha} &\leq \exp{-\frac{3\alpha^2}{6\E{}{g(\bZ)} + 2\alpha}}.\\
%     \mbox{\emph{For every }} 0 < \alpha \leq \E{}{g(\bZ)}, &
%     \P{}{g(\bZ) \leq \E{}{g(\bZ)} - \alpha} &\leq \exp{-\frac{\alpha^2}{2\E{}{g(\bZ)}}}.
% \end{eqnarray*}
% \end{lemma}

% Combining all of the above, we obtain the following concentration result:
% \begin{lemma}[Concentration around $\Psi$]\label{lem:concentration-mab}
%     We have that
%     \begin{eqnarray*}
%         \P{}{\hat{\Psi} - \Psi \geq \frac{1}{3}} &\leq \exp{-\frac{k}{2}}\\
%     \mbox{\emph{For every }} 0 < \alpha \leq \E{}{g(\bZ)}, &
%     \P{}{g(\bZ) \leq \E{}{g(\bZ)} - \alpha} &\leq \exp{-\frac{\alpha^2}{2\E{}{g(\bZ)}}}.
% \end{eqnarray*}
% \end{lemma}

We split the analysis in two cases: Our goal is to upper bound the sum $S$ above (with high probability). Let us name ``clean'' event $\cE = \{|\mu(a) - \barmu_t(a)| \leq r_t(a), \forall a \in [m], t > k\}$. Hence, it suffices to find the $r_t(a)$'s such that $\cE$ holds with high probability. By Hoeffding's bound followed by a union bound over $a$ and $t$, we get that
\begin{align*}
    1 - \P{}{\cE} \leq 2m(T-k) \cdot \exp{-2n_t(a) \cdot r^2_t(a)}
    \leq 2T^2 \cdot \exp{-2n_t(a) \cdot r^2_t(a)} \leq \frac{2}{T^2},
\end{align*}
for which we need $r_t(a) \geq \sqrt{\frac{2\log T}{n_t(a)}}$, for all $t > k$. If event $\cE$ holds, we simultaneously get
\begin{align*}
    &\mu(a^*) - \UCB_t(a^*) = \mu(a^*) - \barmu_t(a^*) - r_t(a^*) \leq 0\\
    &\UCB_t(a_t) - \mu(a_t) = \barmu_t(a_t) - \mu(a_t) + r_t(a_t) \leq 2r_t(a_t).
\end{align*}

\paragraph{Case 1: $0 \leq \Psi \lesssim \log^{-1} T$.} Let us rewrite \Cref{eq:regret-mab} as
\begin{align*}
    R_T(\cA) = -k\Psi &+ \sum_{a \in [m]: \mu(a) < \mu(a^*)} n_{>k}(a) \cdot \Delta(a)\\
    \leq -k\Psi &+ 8\log T \cdot \sum_{a \in [m]: \Delta(a) > } \frac{1}{\Delta(a)} \\
    &+ \sum_{a \in [m]: 0 < \Delta(a) \leq } n_{>k}(a) \cdot \Delta(a).
\end{align*}

\mr{Incomplete.}

% \mr{What we might want to do here is a modification of the above algorithm: If $k \ll \sqrt{mT\log T}$, then we run the previous algorithm. Otherwise, at the end of the first $k$ rounds (which are the same as before), we consider two cases based on the following quantity:
% \begin{align*}
%     \hat{\Psi} := \frac{1}{k} \cdot \left(\sum_{t \leq k} \max_{a \in [m]} x_{a,t} - \max_{a \in [m]} \sum_{t \leq k} x_{a,t}\right),
% \end{align*}
% denoting $\hat{a}$ the arm maximizing the latter term from now on.
% \begin{itemize}
%     \item If $\hat{\Psi} \gtrsim \poly^{-1}(\log T)$, then we run the algorithm presented before;
%     \item Otherwise, we pull arm $\hat{a}$ until the end.
% \end{itemize}
% Here, I expect that $|\hat{\Psi}-\Psi| \leq 2\varepsilon$ with high probability for $k \gtrsim \sqrt{mT\log T}$, where $\varepsilon$ can be as large as $\poly^{-1}(\log T)$. If that's the case, then the previous analysis goes through smoothly up to constants. The other case, i.e., small $\Psi$, also goes through smoothly because we'd have nonpositive regret.}

\paragraph{Case 2: $\Psi \gtrsim \log^{-1} T$.} In this case, to bound $\sum_{t>k} \Delta(a_t)$, we see that
\begin{align*}
    \sum_{t>k} \Delta(a_t) &\leq \sum_{t>k} \left(\mu(a^*) - \UCB_t(a^*)\right) + \left(\UCB_t(a_t) - \mu(a_t)\right) \\
    &\leq 2 \cdot \sum_{t > k} r_t(a_t) = 2 \cdot \sum_{a \in [m]} n_{>k}(a) \cdot r_t(a) = 2\sqrt{2\log T} \cdot \sum_{a \in [m]} \frac{n_{>k}(a)}{\sqrt{n_T(a)}}\\
    &\leq 2\sqrt{2\log T} \cdot \sum_{a \in [m]} \sqrt{n_{>k}(a)} \leq 2\sqrt{2\log T} \cdot m \cdot \sqrt{\frac{1}{m} \cdot \sum_{a \in [m]} n_{>k}(a)}\\
    &\leq 2\sqrt{2m(T-k)\log T},
\end{align*}
where the first inequality follows from observing that $\UCB_t(a_t) \geq \UCB_t(a^*)$ by the way the algorithm works. The second inequality follows from event $\cE$ holding, while the third by observing that $n_{k+1:t}(a) \leq n_t(a)$ for all $t \in [T]$. The fourth inequality follows by Jensen's applied on concave functions (such as $\sqrt{\cdot}$), and the fifth by noticing that $\sum_{a \in [m]} n_{>k}(a) = T-k$.

To compute the final bound on regret, we recall that event $\cE$ does not hold with probability at most $\frac{1}{T^2}$, and the maximum regret in that case is $T$. Overall, we have
\begin{align*}
    R_T(\cA) &= \E{}{R_T(\cA) \mid \cE} \cdot \P{}{\cE} + \E{}{R_T(\cA) \mid \overline{\cE}} \cdot \left(1 - \P{}{\cE}\right)\\
    &\leq 2\sqrt{2mT\log T} - k\Psi + T \cdot \frac{2}{T^2} \leq C,
\end{align*}
which holds as long as $k \gtrsim \frac{\sqrt{mT\log T}}{\Psi}$, for a constant $C \geq 2$. The bicriteria guarantee reads
\[
    (k, R_T) = \left(\tilde{O}(\sqrt{mT}), O(1)\right),
\]
since, in this case, $\Psi \gtrsim \log^{-1} T$.

==> sections/omitted.tex <==
\section{Omitted Proofs}\label{sec:omitted} 

\subsection{Proof of Lemma~\ref{lem:potential-hedge}}

\lempotentialhedge*

\begin{proof}
    We have that, by definition,
    \begin{align*}
        W_{T+1} \geq w_{T+1}(i) 
            w_t(i) \cdot \exp{-\eta\tilde\ell_t(i)} = \prod_{t \in [T]} \exp{-\eta\tilde\ell_t(i)} = \exp{-\eta \tilde L_T(i)}.
    \end{align*}
    We also know that 
    \begin{align*}
        W_{t+1} &\leq W_t \cdot \left(1 - \eta\sum_{i \in [n]} p_t(i)\cdot\tilde\ell_t(i) + \eta^2\sum_{i \in [n]} p_t(i)\cdot\tilde\ell^2_t(i)\right).
    \end{align*}
    Thus,
    \begin{align*}
        W_{T+1} &\leq n \cdot \prod_{t \in [T]} \left(1 - \eta\sum_{i \in [n]} p_t(i) \cdot \tilde\ell_t(i) + \eta^2\sum_{i \in [n]} p_t(i) \cdot \tilde\ell^2_t(i)\right),
    \end{align*}
    which combined with the earlier bound and taking logarithms of both sides, gives
    \begin{align*}
            -\eta\tilde L_T(i) &\leq \log n+\sum_{t \in [T]} \log \left( 1 - \eta\sum_{i \in [n]} p_t(i)\cdot \tilde\ell_t(i) +\eta^2\sum_{i \in [n]} p_t(i) \cdot \tilde\ell^2_t(i) \right)\\
            &\leq \log n - \eta \sum_{t \in [T], i \in [n]} p_t(i) \cdot \tilde\ell_t(i) + \eta^2\sum_{t \in [T], i \in [n]} p_t(i)\cdot \tilde\ell^2_t(i)\\
            &\leq \log n - (\eta - U\eta^2) \sum_{t \in [T], i \in [n]} p_t(i)\cdot \tilde\ell_t(i).
        \end{align*}
    The second inequality above follows from $\log(1+z) \leq z$ for $z \in \R$, and the third by observing that $\tilde\ell^2_t(i) \leq U\tilde\ell_t(i)$, since $\tilde\ell_t(i) \in [0,U]$. The lemma follows by rearranging the terms above.
\end{proof}
